HoneyComb: A Flexible LLM-Based Agent System for Materials Science

The emergence of specialized large language models (LLMs) has shown promise in addressing complex tasks for materials science. Many LLMs, however, often struggle with distinct complexities of material science tasks, such as materials science computational tasks, and often rely heavily on outdated implicit knowledge, leading to inaccuracies and hallucinations. To address these challenges, we introduce HoneyComb, the first LLM-based agent system specifically designed for materials science. HoneyComb leverages a novel, high-quality materials science knowledge base (MatSciKB) and a sophisticated tool hub (ToolHub) to enhance its reasoning and computational capabilities tailored to materials science. MatSciKB is a curated, structured knowledge collection based on reliable literature, while ToolHub employs an Inductive Tool Construction method to generate, decompose, and refine API tools for materials science. Additionally, HoneyComb leverages a retriever module that adaptively selects the appropriate knowledge source or tools for specific tasks, thereby ensuring accuracy and relevance. Our results demonstrate that HoneyComb significantly outperforms baseline models across various tasks in materials science, effectively bridging the gap between current LLM capabilities and the specialized needs of this domain. Furthermore, our adaptable framework can be easily extended to other scientific domains, highlighting its potential for broad applicability in advancing scientific research and applications.

==> sections/intro_v2.tex <==
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{2pt}
      \setlength{\topsep}{2pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1em}   \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em}   \setlength{\itemindent}{0pt}
      \setlength{\listparindent}{0pt}} }

\newcommand{\squishend}{
    \end{list}  }


\section{Introduction}

The emergence of large language models (LLMs) \citep{openai2024, touvron2023llama2, touvron2023llama1} in recent years has led to their application across a wide range of fields including diverse technical fields in science and engineering. This has resulted in a number of new benchmarks measuring the capabilities of language models to perform scientific tasks \citep{wang2023scibench, sun2024scieval, mirza2024large, song-etal-2023-matsci} along with the development of custom LLMs and LLM-based systems for scientific domains including chemistry \citep{bran2023chemcrow, boiko2023autonomous}, biology \citep{Madani_2023} and materials science \citep{miret2024llms, song2023honeybee, gupta2022matscibert, walker2021impact}. 


However, these models often struggle with several significant challenges that hinder their effectiveness. First, they have difficulty performing precise computational tasks, such as determining fluid velocity or molecular mass, due to their inability to utilize external tools to enhance the accuracy of their outputs \cite{zheng2024step}. Second, the content generated by these materials science LLMs is heavily dependent on their internal training data \cite{komeili-etal-2022-internet, liu2024agent}. The high cost of training for these models makes it challenging to continuously update the training datasets. Without regular updates, the accuracy of models diminishes as the underlying data becomes outdated, leading to inaccurate predictions and outputs. This inability to access the latest research on platforms like arXiv or retrieve up-to-date information from Wikipedia further exacerbates the issue, resulting in model outputs that suffer from hallucinations due to outdated or incorrect data.

% Natural Language Processing (NLP) presents a significant potential to expedite the discovery and comprehension of innovative material systems, which is essential for tackling pressing societal issues such as healthcare access and pharmaceutical innovation. The transformative impact of NLP within the realm of materials science is primarily supported by advancements in Large Language Models (LLMs). These developments pave the way for the creation of sophisticated language processing tools that can significantly enhance research endeavors in materials science. In the wake of the burgeoning popularity of LLMs, a plethora of specialized models~\cite{song2023honeybee, gupta2022matscibert, walker2021impact, taylor2022galactica} tailored for the domain of materials science have made their mark, showcasing impressive capabilities in tackling the intricate challenges of this ever-evolving field. 

However, the rapid pace of innovation in materials science demands that existing LLMs remain perpetually updated with the latest findings and discoveries, a requirement that incurs significant training costs and resource investment. The high cost of perpetual training to keep these models updated is compounded by the risk of obsolescence, as outdated data can lead to diminished accuracy and reliability in model predictions~\cite{komeili-etal-2022-internet, liu2024agent}. This is particularly problematic in a field like materials science, where most 
real-world applications, such as material property prediction~\cite{pilania2013accelerating} and calculating fluid dynamics~\cite{lye2020deep}, are not only computationally complex but also require up-to-date and precise information to ensure the validity of outcomes.

Despite the infusion of cutting-edge domain knowledge, LLMs are prone to generating hallucinations when faced with tasks that demand sophisticated inferential capabilities and even the ability to utilize external tools, which is especially true for tasks that require the integration of theoretical understanding with computational precision~\cite{miret2024llms,lee2023matsciml}. As a result, the combination of the latest knowledge, powerful external tools, and LLMs is critical for addressing highly specialized problems that may lie beyond the scope of a plain LLM's capability. 

Considering the aforementioned issues, Augmented Language Models (ALMs)~\cite{mialon2023augmented} have emerged as a promising solution by incorporating external knowledge and tools. This enhances the precision and veracity of LLMs when applied in the material science domain. Different from fine-tuning, which can be employed to calibrate a model within a specific domain, ALMs offer the distinct advantage of enabling the alteration of knowledge sources without necessitating the retraining of the LLMs. This capability not only circumvents the issue of model forgetting but also augments the LLM with a customizable array of external knowledge and tools. 

This paper aims to explore the synergistic potential of combining LLMs with external knowledge and tools for advancing material science, thus we present an LLM-based agent framework named \textit{HoneyComb}. \textit{HoneyComb} encompasses three integral modules meticulously crafted for the domain of materials science: the MatsciKB, the ToolHub, and the Retriever. The MatsciKB module is a highly customized external knowledge base, for which we have specifically engineered a tree-structured framework for knowledge management. This architecture ensures that the knowledge base can be updated promptly and facilitates intuitive human-computer interaction. Regarding the ToolHub, we have curated a suite of tools pertinent to the materials science domain, refactoring them to possess a uniform interface. This standardization not only renders the tools readily accessible for invocation by the LLMs but also diminishes maintenance overheads while enhancing scalability and robustness. As for the Retriever, it operates on a paradigm akin to the recall-rank mechanism of recommendation systems, enabling the model to swiftly pinpoint the requisite knowledge and tools from vast candidates with a balance between precision and efficiency. The key contributions of our research are as follows:

\squishlist
\item The paper introduces \textit{HoneyComb}, a pioneering LLM-based agent system for materials science. To the best of our knowledge, is the first of its kind in the field.
\item The \textit{HoneyComb} integrates the customized knowledge base (MatsciKB) with a knowledge management mechanism, the ToolHub with a standardized tool interface, and an advanced retrieval system (Retriever), all designed to enhance the precision, efficiency, and scalability of materials science research.
\item We conduct experiments on two material science domain datasets. Experimental results show the superiority of our \textit{HoneyComb} framework.




